In search of the weirdest galaxies in the Universe

Weird galaxies are outliers that have either unknown or very uncommon features making them different from the normal sample. These galaxies are very interesting as they may provide new insights into current theories, or can be used to form new theories about processes in the Universe. Interesting outliers are often found by accident, but this will become increasingly more difficult with future big surveys generating an enormous amount of data. This gives the need for machine learning detection techniques to find the interesting weird objects. In this work, we inspect the galaxy spectra of the third data release of the Galaxy And Mass Assembly survey and look for the weird outlying galaxies using two different outlier detection techniques. First, we apply distance-based Unsupervised Random Forest on the galaxy spectra using the flux values as input features. Spectra with a high outlier score are inspected and divided into different categories such as blends, quasi-stellar objects, and BPT outliers. We also experiment with a reconstruction-based outlier detection method using a variational autoencoder and compare the results of the two different methods. At last, we apply dimensionality reduction techniques on the output of the methods to inspect the clustering of similar spectra. We find that both unsupervised methods extract important features from the data and can be used to find many different types of outliers.

==> 0overview.tex <==
\textbf{Quality versus quantity:} use as many words as necessary to describe a difficult problem, but be concise before sounding boring\\

For each paragraph: 
\begin{itemize}
    \item What message do I want to convey? 
    \item What do I expect from results? 
    \item What do I see in the data?
    \item Can I explain what I see?
    \item If not, can I find a reason why it can not be explained?
    \item Don't be to concise in explanation!
\end{itemize}  
\textbf{TENSES FIX AT THE END!}\\

Nice url:\\
\url{https://astrobites.org/guides/galaxy-and-agn-types/}\\


That vs. which\\

can be vs. is \\

we vs. not we\\





















% \section*{Research Outline - Job Formsma}
% \noindent\makebox[\linewidth]{\rule{\linewidth}{0.4pt}}
% \vspace{1cm}

% \underline{Primary goal}:
% \begin{itemize}
%     \item Outlier detection in GAMA DR3 data
% \end{itemize}
% \underline{Expanded goal}:\\
% Inspecting the GAMA DR3 data set \cite{Baldry_2017} of galaxy spectra to look for 
% outliers not earlier reported and inspect the data for errors in, for example, 
% redshift calculations. This is done with unsupervised learning to compute pair-wise 
% similarities between objects. When distances are computed the \textit{distance matrix} 
% can be used for different tasks: outlier detection, visualization using t-SNE 
% or different clustering techniques. \\

% \underline{Methods}:\\
% The primary source for this research is \cite{Baron_2016} where SDSS spectra 
% is ran though a random forest and the highest scoring outliers are inspected 
% visually. This paper shows great results and the algorithm is used again in 
% \cite{Reis_2018a} and \cite{Reis_2018b} to detect more outliers.  We will also
% apply this method and additionally try a more experimentally neural network
% approach to find outliers.\\

% \underline{Research}:
% \begin{enumerate}
%     \item Use the outlier detection algorithm described in \cite{Baron_2016} 
%     and look for outliers in the GAMA DR3 set, find outliers, look at the 
%     'weirdest' galaxies and determine what is weird. Also look for mistakes 
%     in the data where galaxies have wrong parameters, such as redshift (i.e. 
%     due to stars in foreground) or spectra show instrumental errors. As all 
%     data points are used as features, we 
%     can also look at how much (or less) data cleaning is necessary to get good 
%     results. A sample code from \cite{Baron_2016} is available, however the 
%     code is a very basic demo of the concept.
%     \item Visualization on the similarity matrix with tools like t-SNE 
%     as in \cite{Reis_2018a} or UMAP \cite{2018arXiv180203426M}. The structure of 
%     the sample can be projected into a nice 2D map. This can be used to group
%     similar galaxies for easy inspection. 
%     \item Use a different (experimental) novelty detection algorithm, which are
%     mostly described in \cite{PIMENTEL2014215}. This can be compared with the 
%     \cite{Baron_2016} algorithm to compare the outcomes. A good method that we 
%     can try is a Variational Auto Encoder, which can map spectra to a (very) 
%     low dimension and fully reconstruct different types of galaxy spectra as 
%     shown in \cite{SDSSVAE}.
% \end{enumerate}

% \underline{Why?}\\
% This research will give great in sight into the applications of machine learning on 
% high dimensional data such as galaxy spectra. This is a very important topic as
% in the near future very big surveys are taken generating a huge amount of data. 
% With the applied methods we can find outlying galaxies which may have interesting 
% properties. The first method we apply on GAMA data was already proven to work in 
% galaxy spectra. In our work we will look at the details of its application to try 
% to understand the underlying mechanics of the algorithm. A second method using 
% neural networks will be tested. If applied correctly, it is in general better than 
% the already proven method as the training only has to be done once. 
